Veridical Data Science for Medical Foundation Models

The advent of foundation models (FMs) such as large language models (LLMs) has led to a cultural shift in data science, both in medicine and beyond. This shift involves moving away from specialized predictive models trained for specific, well-defined domain questions to generalist FMs pre-trained on vast amounts of unstructured data, which can then be adapted to various clinical tasks and questions. As a result, the standard data science workflow in medicine has been fundamentally altered; the foundation model lifecycle (FMLC) now includes distinct upstream and downstream processes, in which computational resources, model and data access, and decision-making power are distributed among multiple stakeholders. At their core, FMs are fundamentally statistical models, and this new workflow challenges the principles of Veridical Data Science (VDS), hindering the rigorous statistical analysis expected in transparent and scientifically reproducible data science practices. We critically examine the medical FMLC in light of the core principles of VDS: predictability, computability, and stability (PCS), and explain how it deviates from the standard data science workflow. Finally, we propose recommendations for a reimagined medical FMLC that expands and refines the PCS principles for VDS including considering the computational and accessibility constraints inherent to FMs.

==> Citation.tex <==
[1] Rombach R, Blattmann A, Lorenz D, Esser P, Ommer B. High-resolution image synthesis with latent diffusion models. InProceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition 2022 (pp. 10684-10695).

[2] Ramesh A, Pavlov M, Goh G, Gray S, Voss C, Radford A, Chen M, Sutskever I. Zero-shot text-to-image generation. InInternational Conference on Machine Learning 2021 Jul 1 (pp. 8821-8831). PMLR.

[3] Ramesh A, Dhariwal P, Nichol A, Chu C, Chen M. Hierarchical text-conditional image generation with clip latents. arXiv preprint arXiv:2204.06125. 2022 Apr 13.

[4] Ho J, Jain A, Abbeel P. Denoising diffusion probabilistic models. Advances in Neural Information Processing Systems. 2020;33:6840-51.

[5] Song Y, Ermon S. Generative modeling by estimating gradients of the data distribution. Advances in neural information processing systems. 2019;32.

[6] Ho J, Salimans T. Classifier-free diffusion guidance. arXiv preprint arXiv:2207.12598. 2022 Jul 26.

[7] Packhäuser K, Folle L, Thamm F, Maier A. Generation of anonymous chest radiographs using latent diffusion models for training thoracic abnormality classification systems. arXiv preprint arXiv:2211.01323. 2022 Nov 2.

[8] Ali H, Murad S, Shah Z. Spot the fake lungs: Generating synthetic medical images using neural diffusion models. InArtificial Intelligence and Cognitive Science: 30th Irish Conference, AICS 2022, Munster, Ireland, December 8–9, 2022, Revised Selected Papers 2023 Feb 23 (pp. 32-39). Cham: Springer Nature Switzerland.

[9] Chen RJ, Lu MY, Chen TY, Williamson DF, Mahmood F. Synthetic data in machine learning for medicine and healthcare. Nature Biomedical Engineering. 2021 Jun;5(6):493-7.

[10] Lee K, Liu H, Ryu M, Watkins O, Du Y, Boutilier C, Abbeel P, Ghavamzadeh M, Gu SS. Aligning Text-to-Image Models using Human Feedback. arXiv preprint arXiv:2302.12192. 2023 Feb 23.

[11] Feng W, He X, Fu TJ, Jampani V, Akula A, Narayana P, Basu S, Wang XE, Wang WY. Training-Free Structured Diffusion Guidance for Compositional Text-to-Image Synthesis. arXiv preprint arXiv:2212.05032. 2022 Dec 9.

[12] Liu N, Li S, Du Y, Torralba A, Tenenbaum JB. Compositional visual generation with composable diffusion models. InComputer Vision–ECCV 2022: 17th European Conference, Tel Aviv, Israel, October 23–27, 2022, Proceedings, Part XVII 2022 Oct 24 (pp. 423-439). Cham: Springer Nature Switzerland.

[13] Ziegler DM, Stiennon N, Wu J, Brown TB, Radford A, Amodei D, Christiano P, Irving G. Fine-tuning language models from human preferences. arXiv preprint arXiv:1909.08593. 2019 Sep 18.

[14] Stiennon N, Ouyang L, Wu J, Ziegler D, Lowe R, Voss C, Radford A, Amodei D, Christiano PF. Learning to summarize with human feedback. Advances in Neural Information Processing Systems. 2020;33:3008-21.

[15] Song Y, Durkan C, Murray I, Ermon S. Maximum likelihood training of score-based diffusion models. Advances in Neural Information Processing Systems. 2021 Dec 6;34:1415-28.

[16] Kingma DP, Welling M. Auto-encoding variational bayes. arXiv preprint arXiv:1312.6114. 2013 Dec 20.

[17] Goodfellow I, Pouget-Abadie J, Mirza M, Xu B, Warde-Farley D, Ozair S, Courville A, Bengio Y. Generative adversarial networks. Communications of the ACM. 2020 Oct 22;63(11):139-44.

[18] Sohl-Dickstein J, Weiss E, Maheswaranathan N, Ganguli S. Deep unsupervised learning using nonequilibrium thermodynamics. InInternational Conference on Machine Learning 2015 Jun 1 (pp. 2256-2265). PMLR.

[19] Dhariwal, Prafulla, and Alexander Nichol. "Diffusion models beat gans on image synthesis." Advances in Neural Information Processing Systems 34 (2021): 8780-8794.

[20] Müller-Franzes G, Niehues JM, Khader F, Arasteh ST, Haarburger C, Kuhl C, Wang T, Han T, Nebelung S, Kather JN, Truhn D. Diffusion Probabilistic Models beat GANs on Medical Images. arXiv preprint arXiv:2212.07501. 2022 Dec 14.

[21] Pinaya WH, Tudosiu PD, Dafflon J, Da Costa PF, Fernandez V, Nachev P, Ourselin S, Cardoso MJ. Brain imaging generation with latent diffusion models. InDeep Generative Models: Second MICCAI Workshop, DGM4MICCAI 2022, Held in Conjunction with MICCAI 2022, Singapore, September 22, 2022, Proceedings 2022 Oct 8 (pp. 117-126). Cham: Springer Nature Switzerland.

[22] Khader F, Mueller-Franzes G, Arasteh ST, Han T, Haarburger C, Schulze-Hagen M, Schad P, Engelhardt S, Baessler B, Foersch S, Stegmaier J. Medical Diffusion--Denoising Diffusion Probabilistic Models for 3D Medical Image Generation. arXiv preprint arXiv:2211.03364. 2022 Nov 7.

[23] Kazerouni A, Aghdam EK, Heidari M, Azad R, Fayyaz M, Hacihaliloglu I, Merhof D. Diffusion models for medical image analysis: A comprehensive survey. arXiv preprint arXiv:2211.07804. 2022 Nov 14.

[24] Chow LS, Paramesran R. Review of medical image quality assessment. Biomedical signal processing and control. 2016 May 1;27:145-54.

[25] Ho J, Salimans T. Classifier-free diffusion guidance. arXiv preprint arXiv:2207.12598. 2022 Jul 26.

[26] Radford A, Kim JW, Hallacy C, Ramesh A, Goh G, Agarwal S, Sastry G, Askell A, Mishkin P, Clark J, Krueger G. Learning transferable visual models from natural language supervision. InInternational conference on machine learning 2021 Jul 1 (pp. 8748-8763). PMLR.

[27] Raffel C, Shazeer N, Roberts A, Lee K, Narang S, Matena M, Zhou Y, Li W, Liu PJ. Exploring the limits of transfer learning with a unified text-to-text transformer. The Journal of Machine Learning Research. 2020 Jan 1;21(1):5485-551.

[28] Gatys LA, Ecker AS, Bethge M. A neural algorithm of artistic style. arXiv preprint arXiv:1508.06576. 2015 Aug 26.

[29] Dong C, Loy CC, He K, Tang X. Image super-resolution using deep convolutional networks. IEEE transactions on pattern analysis and machine intelligence. 2015 Jun 1;38(2):295-307.

[30] Bakas S, Akbari H, Sotiras A, Bilello M, Rozycki M, Kirby JS, Freymann JB, Farahani K, Davatzikos C. Advancing the cancer genome atlas glioma MRI collections with expert segmentation labels and radiomic features. Scientific data. 2017 Sep 5;4(1):1-3.

[31] Gupta R, Kurc T, Sharma A, Almeida JS, Saltz J. The emergence of pathomics. Current Pathobiology Reports. 2019 Sep 15;7:73-84.

[32] Chen RJ, Lu MY, Wang J, Williamson DF, Rodig SJ, Lindeman NI, Mahmood F. Pathomic fusion: an integrated framework for fusing histopathology and genomic features for cancer diagnosis and prognosis. IEEE Transactions on Medical Imaging. 2020 Sep 3;41(4):757-70.

[33] Ali H, Murad S, Shah Z. Spot the fake lungs: Generating synthetic medical images using neural diffusion models. InArtificial Intelligence and Cognitive Science: 30th Irish Conference, AICS 2022, Munster, Ireland, December 8–9, 2022, Revised Selected Papers 2023 Feb 23 (pp. 32-39). Cham: Springer Nature Switzerland.

[34] Khader F, Mueller-Franzes G, Arasteh ST, Han T, Haarburger C, Schulze-Hagen M, Schad P, Engelhardt S, Baessler B, Foersch S, Stegmaier J. Medical Diffusion--Denoising Diffusion Probabilistic Models for 3D Medical Image Generation. arXiv preprint arXiv:2211.03364. 2022 Nov 7.

[35] Pinaya WH, Tudosiu PD, Dafflon J, Da Costa PF, Fernandez V, Nachev P, Ourselin S, Cardoso MJ. Brain imaging generation with latent diffusion models. InDeep Generative Models: Second MICCAI Workshop, DGM4MICCAI 2022, Held in Conjunction with MICCAI 2022, Singapore, September 22, 2022, Proceedings 2022 Oct 8 (pp. 117-126). Cham: Springer Nature Switzerland.

[36] Müller-Franzes G, Niehues JM, Khader F, Arasteh ST, Haarburger C, Kuhl C, Wang T, Han T, Nebelung S, Kather JN, Truhn D. Diffusion Probabilistic Models beat GANs on Medical Images. arXiv preprint arXiv:2212.07501. 2022 Dec 14.

[37] Bahdanau D, Cho K, Bengio Y. Neural machine translation by jointly learning to align and translate. arXiv preprint arXiv:1409.0473. 2014 Sep 1.

[38] Kreutzer J, Khadivi S, Matusov E, Riezler S. Can neural machine translation be improved with user feedback?. arXiv preprint arXiv:1804.05958. 2018 Apr 16.

[39] Nakano R, Hilton J, Balaji S, Wu J, Ouyang L, Kim C, Hesse C, Jain S, Kosaraju V, Saunders W, Jiang X. Webgpt: Browser-assisted question-answering with human feedback. arXiv preprint arXiv:2112.09332. 2021 Dec 17.

[40] MacGlashan J, Ho MK, Loftin R, Peng B, Wang G, Roberts DL, Taylor ME, Littman ML. Interactive learning from policy-dependent human feedback. InInternational Conference on Machine Learning 2017 Jul 17 (pp. 2285-2294). PMLR.

[41] Lee K, Smith L, Abbeel P. Pebble: Feedback-efficient interactive reinforcement learning via relabeling experience and unsupervised pre-training. arXiv preprint arXiv:2106.05091. 2021 Jun 9.

[42] Ouyang, L., Wu, J., Jiang, X., Almeida, D., Wainwright, C. L., Mishkin, P., Zhang, C., Agarwal, S., Slama, K., Ray, A., et al. Training language models to follow instructions with human feedback. arXiv preprint arXiv:2203.02155, 2022.

[43] Bai, Y., Jones, A., Ndousse, K., Askell, A., Chen, A., DasSarma, N., Drain, D., Fort, S., Ganguli, D., Henighan, T., et al. Training a helpful and harmless assistant with reinforcement learning from human feedback. arXiv preprint arXiv:2204.05862, 2022a. 

[44] Bai, Y., Kadavath, S., Kundu, S., Askell, A., Kernion, J., Jones, A., Chen, A., Goldie, A., Mirhoseini, A., McKinnon, C., et al. Constitutional ai: Harmlessness from ai feedback. arXiv preprint arXiv:2212.08073, 2022b.

==> preamble/minimalist_biblatex.tex <==
\usepackage[%
minnames=1,maxnames=99,maxcitenames=2,
style=alphabetic,
doi=false,
url=false,
firstinits=true,
hyperref,
natbib,
backend=bibtex,
sorting=nyt
]{biblatex}%

\newbibmacro*{journal}{%
  \iffieldundef{journaltitle}
    {}
    {\printtext[journaltitle]{%
       \printfield[noformat]{journaltitle}%
       \setunit{\subtitlepunct}%
       \printfield[noformat]{journalsubtitle}}}}

%\DeclareFieldFormat[article,inbook,incollection,inproceedings,patent,thesis,unpublished]{titlecase}{\MakeSentenceCase*{#1}}
% print the title of articles and any in* type entry in sentence case
\DeclareFieldFormat{sentencecase}{\MakeSentenceCase*{#1}}

\renewbibmacro*{title}{%
  \ifthenelse{\iffieldundef{title}\AND\iffieldundef{subtitle}}
    {}
    {\ifthenelse{\ifentrytype{article}\OR\ifentrytype{inbook}%
      \OR\ifentrytype{incollection}\OR\ifentrytype{inproceedings}%
      \OR\ifentrytype{inreference}}
      {\printtext[title]{%
        \printfield[sentencecase]{title}%
        \setunit{\subtitlepunct}%
        \printfield[sentencecase]{subtitle}}}%
      {\printtext[title]{%
        \printfield[titlecase]{title}%
        \setunit{\subtitlepunct}%
        \printfield[titlecase]{subtitle}}}%
     \newunit}%
  \printfield{titleaddon}}



\AtEveryBibitem{%
\ifentrytype{article}{
    \clearfield{url}%
    \clearfield{urldate}%
    \clearfield{eprint}
    \clearfield{eid}
}{}
\ifentrytype{book}{
    \clearfield{url}%
    \clearfield{urldate}%
}{}
\ifentrytype{collection}{
    \clearfield{url}%
    \clearfield{urldate}%
}{}
\ifentrytype{incollection}{
    \clearfield{url}%
    \clearfield{urldate}%
}{}
}

\AtEveryBibitem{
    \clearfield{pages}
    \clearfield{review}%
    \clearfield{series}%%
    \clearfield{volume}
    \clearfield{month}
    \clearfield{eprint}
    \clearfield{isbn}
    \clearfield{issn}
    \clearlist{location}
    \clearfield{series}
    \clearlist{publisher}
    \clearname{editor}
}{}

==> preamble/nocommenting.tex <==
\newcommand{\LATER}[1]{\error}
\newcommand{\fLATER}[1]{\error}
\newcommand{\TBD}[1]{\error}
\newcommand{\fTBD}[1]{}
\newcommand{\PROBLEM}[1]{\error}
\newcommand{\fPROBLEM}[1]{\error}
\newcommand{\NA}[1]{#1} 


==> preamble/preamble.tex <==
%\RequirePackage[l2tabu, orthodox]{nag}

% FONTS
\usepackage[utf8]{inputenc} % allow utf-8 input
\usepackage[T1]{fontenc}    % use 8-bit T1 fonts

% Replace default Latin Modern typewriter with its proportional counterpart
% http://www.tug.dk/FontCatalogue/lmoderntypewriterprop/
\renewcommand*\ttdefault{lmvtt}


%%% OPTION 1 - Fourier Math + New Century Schoolbook + ParaType Sans

% % Import Fourier Math (this imposes its own New Century Schoolbook type)
% % http://www.ctan.org/tex-archive/fonts/fouriernc/
% \usepackage{fouriernc}
% \usepackage{amsmath}
% % Replace with TeX Gyre Schola version of New Century Schoolbook (must scale!)
% % http://www.tug.dk/FontCatalogue/tgschola/
% \usepackage[scale=0.92]{tgschola}
% \usepackage[scaled=0.88]{PTSans}

%% OPTION 2 - MathDesign Math + Bitstream Charter + ParaType Sans

% Import MathDesign (this brings along Bitstream Charter)
% http://www.ctan.org/tex-archive/fonts/mathdesign/
\usepackage[bitstream-charter]{mathdesign}
\usepackage{amsmath}
\usepackage[scaled=0.92]{PTSans}


% %%% OPTION 3 - MTPRO 2 Math + Termes Times + ParaType Sans

% \usepackage{tgtermes}
% \usepackage{amsmath}
% \usepackage[subscriptcorrection,
%             amssymbols,
%             mtpbb,
%             mtpcal,
%             nofontinfo  % suppresses all warnings
%            ]{mtpro2}
% \usepackage{scalefnt,letltxmacro}
% \LetLtxMacro{\oldtextsc}{\textsc}
% \renewcommand{\textsc}[1]{\oldtextsc{\scalefont{1.10}#1}}
% \usepackage[scaled=0.92]{PTSans}

% GEOMETRY
\usepackage[
  paper  = letterpaper,
  left   = 1.65in,
  right  = 1.65in,
  top    = 1.0in,
  bottom = 1.0in,
  ]{geometry}

% COLOR
\usepackage[usenames,dvipsnames,table]{xcolor}
%\usepackage[usenames,table]{xcolor}
\definecolor{shadecolor}{gray}{0.9}

% SPACING and TEXT
\usepackage[final,expansion=alltext]{microtype}
\usepackage[english]{babel}
\usepackage[parfill]{parskip}
\usepackage{afterpage}
\usepackage{framed}

%redefine the leftbar environment to accept a width and coloring options
\renewenvironment{leftbar}[1][\hsize]
{%
  \def\FrameCommand
  {%
    {\color{Gray}\vrule width 3pt}%
    \hspace{10pt}%
    %\hspace{0pt}\fboxsep=\FrameSep\colorbox{black!10}%
  }%
  \MakeFramed{\hsize#1\advance\hsize-\width\FrameRestore}%
}%
{\endMakeFramed}

% define a paragraph header function
\DeclareRobustCommand{\parhead}[1]{\textbf{#1}~}

% EDITING
% line numbering in left margin
\usepackage{lineno}
\renewcommand\linenumberfont{\normalfont
                             \footnotesize
                             \sffamily
                             \color{SkyBlue}}
% ragged paragraphs in right margin
\usepackage{ragged2e}
\DeclareRobustCommand{\sidenote}[1]{\marginpar{
                                    \RaggedRight
                                    \textcolor{Plum}{\textsf{#1}}}}
% paragraph counter in right margin
\newcommand{\parnum}{\bfseries\P\arabic{parcount}}
\newcounter{parcount}
\newcommand\p{%
    \stepcounter{parcount}%
    \leavevmode\marginpar[\hfill\parnum]{\parnum}%
}
% paragraph helper
\DeclareRobustCommand{\PP}{\textcolor{Plum}{\P} }

% COUNTERS
\renewcommand{\labelenumi}{\color{black!67}{\arabic{enumi}.}}
\renewcommand{\labelenumii}{{\color{black!67}(\alph{enumii})}}
\renewcommand{\labelitemi}{{\color{black!67}\textbullet}}

% FIGURES
\usepackage{graphicx}
\usepackage{wrapfig}
\usepackage[labelfont=bf,font=footnotesize,width=.9\textwidth]{caption}
\usepackage[format=hang]{subcaption}

% TABLES
\usepackage{booktabs,multirow,multicol}       % professional-quality tables

% ALGORITHMS
\usepackage[algoruled]{algorithm2e}
\usepackage{listings}
\usepackage{fancyvrb}
\fvset{fontsize=\normalsize}

% BIBLIOGRAPHY
%\usepackage{natbib}

% HYPERREF
\usepackage[colorlinks,linktoc=all]{hyperref}
\usepackage[all]{hypcap}
\hypersetup{citecolor=MidnightBlue}
\hypersetup{linkcolor=MidnightBlue}
\hypersetup{urlcolor=MidnightBlue}

% CLEVEREF must come after HYPERREF
\usepackage[nameinlink]{cleveref}

% ACRONYMS
\usepackage[acronym,smallcaps,nowarn]{glossaries}
% \makeglossaries

% COLOR DEFINITIONS
\newcommand{\red}[1]{\textcolor{BrickRed}{#1}}
\newcommand{\orange}[1]{\textcolor{BurntOrange}{#1}}
\newcommand{\green}[1]{\textcolor{OliveGreen}{#1}}
\newcommand{\blue}[1]{\textcolor{MidnightBlue}{#1}}
\newcommand{\gray}[1]{\textcolor{black!60}{#1}}

% LISTINGS DEFINTIONS
\lstdefinestyle{mystyle}{
    commentstyle=\color{OliveGreen},
    keywordstyle=\color{BurntOrange},
    numberstyle=\tiny\color{black!60},
    stringstyle=\color{MidnightBlue},
    basicstyle=\ttfamily,
    breakatwhitespace=false,
    breaklines=true,
    captionpos=b,
    keepspaces=true,
    numbers=left,
    numbersep=5pt,
    showspaces=false,
    showstringspaces=false,
    showtabs=false,
    tabsize=2
}
\lstset{style=mystyle}

